Competitive Equilibria with Unequal Budgets: Supporting Arbitrary Pareto Optimal Allocations

We consider a market setting of agents with additive valuations over heterogeneous divisible resources. Agents are assigned a budget of tokens (possibly unequal budgets) they can use to obtain resources; leftover tokens are worthless. We show how to support any Pareto efficient allocation in equilibrium, using anonymous resource prices and agent specific budgets. We also give computationally efficient algorithms for those tasks. In particular, this allows us to support the Rawlsian max-min allocation.

==> special-cases.tex <==
\subsection{faster computation of max-min allocations}

The computation of the max-min allocation, as well the item pricing scheme require solving linear programs, which although efficient, may still be time consuming. If the number of agents or items is small, it is possible to compute the allocation, prices and budgets more efficiently.

\subsubsection{2 agents, $m$ items} \label{two agents}

For each item $j$ define $\phi_j=v_{2,j}/v_{1,j}$, and we sort the items by $\phi_j$.
Let $\pi$ be a permutation of $1,\ldots,m$ such that $\phi_{\pi_j} \leq \phi_{\pi_{j+1}}$ for $j=1,\ldots, m-1$. For simplicity we assume that $\pi_j = j$.


Agent $1$ is assigned (fractional) items in the order $\phi_{1}, \phi_{2}, \ldots$ whereas agent 2 is assigned items in the order $\phi_{m}, \phi_{m-1}, \ldots$.
We simultaneously increase the allocations for both agents, so that the valuations to the two agents are equal, until the two thresholds meet, producing a partition of the items. The infinitesimal rate at which the value for agent 1 increases is set to be equal to the infinitesimal rate at which the value for agent 2 increases.

{\sl I.e.}, we find a ``median" item. Namely, an index $s$ such that
$\sum_{j=1}^s v_{1,j} \geq \sum_{j=s+1}^m v_{2,j}$ and
$\sum_{j=1}^{s-1} v_{1,i} \leq \sum_{j=s}^m v_{2,j}$.

Except for possibly one item, (item $s$), other items are assigned in their entirety to one of the two agents. Let this {\sl max min} allocation be denoted $\widehat{x}_{i,j}$, where $\widehat{x}_i = \widehat{x}_{i,1}, \widehat{x}_{i,3}, \ldots, \widehat{x}_{i,m}$ for $i=1,2$. Note that
$$\widehat{x}_{1}= 1,1,\ldots,1, x_{1,s}, 0,\ldots,0\mbox{\rm\ whereas\ }\widehat{x}_{2}= 0,0,\ldots,0, 1-x_{1,s}, 1,\ldots,1.$$ A simple algorithm for computing such a max min allocation, $\widehat{x}$, is to search for some $s$ such that item $s$ can be partitioned in such a way that the value of the allocation for agent 1 is equal to the value of the allocation for agent 2.

Item $j$ is priced at $p_j=v_{1,j}$. The budget for agent $1$ is set to $b_1=\sum_j \widehat{x}_{1,j} v_{1,j}$. We now argue that  $\widehat{x}_{1}$ is in the demand set of agent $1$.
The value per token for agent $1$ is equal across all items, therefore the agent is indifferent as to which items are chosen, as long as the prices add up to $b_1$ and may as well be happy with the items with values in increasing order of $v_{2,j}/v_{1,j}$.

The budget for agent $2$, is set to be $b_2=\sum_j p_j x_{2,j} = \sum_j v_{1,j} x_{2,j}$. Again, we need to show that $\widehat{x}_2$ is in the demand set of Agent 2. Agent 2 greedily prefers to use her budget on items with the largest $v_{2,j}/p_j$.  She is assigned the items in order of decreasing $v_{2,j}/p_j=v_{2,j}/v_{1,j}$. Ergo, $x_{2}$ is in the demand set of agent $2$.

\ymnote{There are alternative prices and budgets that would work equally well. It seems that the pricing $p_j=\max(v_{1,j},v_{2,j})$ works and there may be others.}

\subsubsection{ $n$ agents, 2 items}

Order the agents in decreasing order of $\rho_i=v_{i,1}/v_{i,2}$. Similarly to subsection \ref{two agents}, without loss of generality we assume the indices are already ordered, i.e. $\rho_i\leq \rho_{i+1}$, $i=1,\ldots,n$.

The goal is to assign fractions of item {1} to agents with larger $\rho_i$ and fractions of item {2} to agents with smaller $\rho_i$. Agents will get equal value from their shares. There may be some agent, agent $k$, that gets non zero parts of both items.

Define variables $x_{i,1}, x_{i,2}$, $i=1,\ldots,n$. We seek a value of $k$ and a solution to the following equations:
\begin{eqnarray}
                    x_{i,j}&\geq& 0; \qquad i=1,\ldots,n; \quad j=1,2 \label{eq:init1} \\
                    x_{1,2}=\cdots = x_{k-1,2} = x_{k+1,1}=\cdots =x_{n,1}&=& 0 \label{eq:init2} \\
                  x_{1,1}+x_{2,1}+\cdots+x_{k-1,1} + x_{k,1} &=& 1 \label{eq:equal1} \\
                                   x_{k,2}+x_{k+1,2}+\cdots+x_{n,2} &=& 1 \label{eq:equal2}\\
                                  x_{1,1}v_{1,1} = x_{2,1}v_{2,1} = \cdots =x_{k-1,1}v_{k-1,1} &=& x_{k,1}v_{k,1} + x_{k,2}v_{k,2}\label{eq:subs}\\ &=& x_{k+1,2}v_{k+1,2} = x_{k+2,2}v_{k+2,2} = \cdots =x_{n,2}v_{n,2}\nonumber
\end{eqnarray}

% Using Equation \ref{eq:subs} and  we derive that $$x_{1,1}=\frac{ x_{k,1}v_{k,1} + x_{k,2}v_{k,2}}{v_{1,1}},  \ldots, x_{k-1,1}=\frac{ x_{k,1}v_{k,1} + x_{k,2}v_{k,2}}{v_{k-1,1}},$$ and $$x_{k+1,1}=\frac{ x_{k,1}v_{k,1} + x_{k,2}v_{k,2}}{v_{k+1,1}},  \ldots, x_{n,1}=\frac{ x_{k,1}v_{k,1} + x_{k,2}v_{k,2}}{v_{n,1}}.$$
%
% Substituting these equalities into equations \ref{eq:equal1} and \ref{eq:equal2} we get two equations and two variables, and can solve for $x_{k,1}$ and $x_{k,2}$. This defines all $x_{i,j}$ and we can check that the conditions hold.
% It remains to show that there exists some such $k$.


 Given such a solution, we set $p_1=v_{k,1}$ and $p_2=v_{k,2}$. This means that agent $k$ is indifferent between equal sized parts of items 1 and 2, whereas all agents $i<k$ prefer equal sized parts of item $1$ over the same sized parts of item $2$, and vice-versa for agents $i>k$.

 Agents $i \in 1,\ldots,k-1$ receive budget $b_i = x_{i, 1} p_1$. Agents $i \in k+1,\ldots,n$ receive budget $b_i = x_{i, 2} p_2$. The $k$-th agent's bedget is $b_k = x_{k, 1} p_1 + x_{k, 2} p_2$.
  All agents $i<k$ can afford an $x_{i,1}$ fraction of item 1, the item does not run out, and this is in their demand set. Likewise for agents $i>k$ (with respect to item 2). Agent $k$ gets the leftovers from both items, $x_{k,1}$ fraction of item 1 and $x_{k,2}$ fraction of item 2, which is in her demand set.

  Actually, the linear program in (\ref{eq:init1}, \ref{eq:init2}, \ref{eq:equal1}, \ref{eq:equal2}) defines all of the Pareto optimal allocations. Since the Linear program of the max-min optimization has a solution, and there is a max-min solution that is Pareto optimal, there must exist an agent $k$ for which there is a solution.

  Instead of solving the linear program directly for each possible value of $k$, one can directly solve equations \ref{eq:init2}, \ref{eq:equal1}, \ref{eq:equal2} and \ref{eq:subs}, searching for a value of $k$ for which a feasible solution exists that also satisfies the constraints in \ref{eq:init1}.

  \nanotenew{perhaps the Pareto optimality claim, although trivial, should be explained. Each agent receives a fraction of her "preferred" item (not necessarily preferred in net valuation, but preferred relatively to the preferences of the agents that get the other item), and both items are fully allocated.}

